Reweighting Strategy based on Synthetic Data Identification for Sentence Similarity

Semantically meaningful sentence embeddings are important for numerous tasks in natural language processing. To obtain such embeddings, recent studies explored the idea of utilizing synthetically generated data from pretrained language models (PLMs) as a training corpus. However, PLMs often generate sentences much different from the ones written by human. We hypothesize that treating all these synthetic examples equally for training deep neural networks can have an adverse effect on learning semantically meaningful embeddings. To analyze this, we first train a classifier that identifies machine-written sentences, and observe that the linguistic features of the sentences identified as written by a machine are significantly different from those of human-written sentences. Based on this, we propose a novel approach that first trains the classifier to measure the importance of each sentence. The distilled information from the classifier is then used to train a reliable sentence embedding model. Through extensive evaluation on four real-world datasets, we demonstrate that our model trained on synthetic data generalizes well and outperforms the existing baselines. Our implementation is publicly available at https://github.com/ddehun/coling2022_reweighting_sts.

==> table3.tex <==
\begin{table*}[t]
\centering
    \footnotesize
    \begin{adjustbox}{width=1.0\textwidth}
        \begin{tabular}{clccccccc}
            \toprule
              &  & \multicolumn{2}{c}{\textbf{STSb}} & \multicolumn{2}{c}{\textbf{QQP}} & \multicolumn{2}{c}{\textbf{MRPC}} & \multicolumn{1}{c}{\textbf{PAWS}}  \\ \cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-9} 
            $C_{src}$ & \textbf{Model} & \multicolumn{1}{c}{$r$} & \multicolumn{1}{c}{$\rho$}  & \multicolumn{1}{c}{Acc.} & \multicolumn{1}{c}{F1}    & \multicolumn{1}{c}{Acc.} & \multicolumn{1}{c}{F1}    & \multicolumn{1}{c}{F1}        \\ \midrule
            % &\multicolumn{15}{l}{\textit{\textbf{Supervised}}}\\ \hline
            % &GloVe          
            % &47.30	&50.70	&68.51	&	63.30	&	71.53	&	80.91	&	44.16 \\ 
            % &BERT-CLS           
            % &17.18	&20.30	&66.38	&	61.50	&	66.03	&	79.79	&	49.32 \\ 
            % &BERT       
            % &47.91	&47.29	&68.70	&	64.26	&	70.38	&	80.50	&	46.05	\\
            % &BERT*           
            % &74.15	&76.98	&73.10	&	67.08	&	73.39	&	81.68	&	53.91	\\ 
            % &RoBERTa        
            % &52.36	&54.35	&67.91	&	63.67	&	72.28	&	81.20	&	44.03	\\ 
            % &RoBERTa*        
            % & 74.78	&77.80	&73.56	&	67.00	&	\underline{75.76}&	\underline{82.46}	&	\underline{56.48}\\ 
            % &USE*            
            % & 78.72	&77.08	&73.19	&	\underline{69.27}&	67.47	&	80.35	&	45.34	\\
            % &InferSent*      
            % &49.53	&50.86	&68.94	&	64.13	&	65.97	&	79.32	&45.01	\\ 
            % \hline
            \multirow{2}{*}{\textit{\textbf{STSb}}}
            &DINO     
            &78.45&77.71&73.14&	68.04&	70.44	&81.16&	47.30\\ 
            &RISE      
            & \textbf{79.11}	{\scriptsize (+0.66)}&	\textbf{78.57}	{\scriptsize (+0.86)}&	\textbf{74.47}	{\scriptsize (+1.33)}&	\textbf{69.08}	{\scriptsize (+1.04)}&	\textbf{72.84}	{\scriptsize (+2.4)}&	\textbf{82.01}	{\scriptsize (+0.85)}&	\textbf{50.24}	{\scriptsize (+2.94)} \\
            &$\llcorner$ {\scriptsize Filtering}
            & 77.73	{\scriptsize (-0.72)}&	77.45	{\scriptsize (-0.26)}&	73.06	{\scriptsize (-0.08)}&	67.94	{\scriptsize (-0.10)}&	68.96	{\scriptsize (-1.48)}&	81.35	{\scriptsize (+0.19)}&	46.72	{\scriptsize (-0.58)}\\
            &$\llcorner$ {\scriptsize Random}
            & 79.03	{\scriptsize (+0.58)}	&78.39	{\scriptsize (+0.68)}&	73.09	{\scriptsize (-0.05)}&	68.03	{\scriptsize (-0.01)}&	71.09	{\scriptsize (+0.65)}&	81.62	{\scriptsize (+0.46)} &50.17	{\scriptsize (+2.87)}\\
            \hline
            % % %
            \multirow{2}{*}{\textit{\textbf{QQP}}} 
            &DINO      
            & 64.93&	65.93&	73.20&	67.72&	70.75&	80.40&44.47	\\ 
            &RISE 
            & \textbf{78.36}	{\scriptsize (+13.43)}&	\textbf{77.13}	{\scriptsize (+11.2)}&	73.35	{\scriptsize (+0.15)}&	67.76	{\scriptsize (+0.04)}&	\textbf{72.38}	{\scriptsize (+1.63)}&	\textbf{81.35}	{\scriptsize (+0.95)}&	46.28	{\scriptsize (+1.81 )}\\
            
            &$\llcorner$ {\scriptsize Filtering}
            &65.24	{\scriptsize (+0.31)}&	66.36	{\scriptsize (+0.43)}&	\textbf{73.48}	{\scriptsize (+0.28)}	&\textbf{67.95}	{\scriptsize (+0.23)}	&69.77	{\scriptsize (-0.98)}&	80.26	{\scriptsize (-0.14)}&	43.36	{\scriptsize (-1.11)}\\
            % &$\llcorner$ {\scriptsize Shuffling}
            % &65.34	{\scriptsize (+0.41)}&	66.43	{\scriptsize (+0.50)}	&73.8	{\scriptsize (+0.6)}	&\textbf{68.24}	{\scriptsize (+0.52)}&	69.78	{\scriptsize (-0.97)}	&80.82	{\scriptsize (+0.42)}&	42.42	{\scriptsize (-2.05)}\\
            &$\llcorner$ {\scriptsize Random}
            & 73.49	{\scriptsize (+8.56)}&	72.88	{\scriptsize (+6.95)}&	73.14	{\scriptsize (-0.06)}&	67.75	{\scriptsize (+0.03)}&69.76	{\scriptsize (-0.99)}&	80.83{\scriptsize (	+0.43)}&	\textbf{46.97}	{\scriptsize (+2.5)}\\
            \hline
            
            % % %
            \multirow{2}{*}{\textit{\textbf{MRPC}}}
            &DINO     
            & 75.51	&	73.87&	71.85&	65.70		&71.57	&81.55&	47.35\\
            &RISE      
            & \textbf{77.47}	{\scriptsize (+1.96)}&	\textbf{76.86}	{\scriptsize (+2.99)}&	\textbf{74.23}	{\scriptsize (+2.38)}&	\textbf{68.82}	{\scriptsize (+3.12)}	&71.97	{\scriptsize (+0.4)} &	\textbf{81.95}	{\scriptsize (+0.4)}	&\textbf{49.35}	{\scriptsize (+2.00)} \\
            &$\llcorner$ {\scriptsize Filtering}
            &76.25	{\scriptsize (+0.74)}&	74.88	{\scriptsize (+1.01)}&	71.05	{\scriptsize (-0.80)}&	64.82	{\scriptsize (-0.88)}&	71.34	{\scriptsize (-0.23)}&	80.76	{\scriptsize (-0.79)}&	47.84	{\scriptsize (+0.49)}\\
            % &$\llcorner$ {\scriptsize Shuffling}
            % & 74.07	{\scriptsize (-1.44)}	&72.44	{\scriptsize (-1.43)}&	71.98	{\scriptsize (+0.13)}&	65.96	{\scriptsize (+0.26)}&	71.21	{\scriptsize (-0.36)}&	80.87	{\scriptsize (-0.68)}&	47.58	{\scriptsize (+0.23)}\\
            &$\llcorner$ {\scriptsize Random}
            & 76.06	{\scriptsize (+0.55)}&	74.51	{\scriptsize (+0.64)}&	72.52	{\scriptsize (+0.67)}&	66.45	{\scriptsize (+0.75)}&	\textbf{72.19}	{\scriptsize (+0.62)}&	81.71	{\scriptsize (+0.16)}&	47.56	{\scriptsize (+0.21)}\\
            
            \bottomrule
            % 각 데이터셋 컬럼 합치고 데이터셋 이름 넣고 선 굵게
        \end{tabular}
    \end{adjustbox}
    \vspace{-3mm}
    \caption{Evaluation results of different sentence embedding models on four sentence similarity task dataset. We highlight the best result within each $C_{src}$ in each metric as \textbf{bold}. The number in right bracket indicates the performance difference with DINO. For regression task, we use Pearson correlation~($r$) and Spearman's rank correlation coefficient~($\rho$) metrics are used for evaluation. Each score represents the average of five trials.}
    \vspace{-2mm}
    \label{tab:main}
\end{table*}

